Statistical Model Checking : An Overview

Quantitative properties of stochastic systems are usually specified in logics that allow one to compare the measure of executions satisfying certain temporal properties with thresholds. The model checking problem for stochastic systems with respect to such logics is typically solved by a numerical approach that iteratively computes (or approximates) the exact measure of paths satisfying relevant subformulas; the algorithms themselves depend on the class of systems being analyzed as well as the logic used for specifying the properties. Another approach to solve the model checking problem is to \emph{simulate} the system for finitely many runs, and use \emph{hypothesis testing} to infer whether the samples provide a \emph{statistical} evidence for the satisfaction or violation of the specification. In this short paper, we survey the statistical approach, and outline its main advantages in terms of efficiency, uniformity, and simplicity.

==> next.tex <==
\section{Where shall we go next?}

We identify several directions to extend the applicability of
statistical model checking techniques.

\begin{itemize}
\item
Using efficient techniques for performing simulation is crucial to
guarantee good performances for any statistical model checking
algorithm. Unfortunately, the existing algorithms do not efficient
simulation techniques. It would thus be worth combining statistical
model checking algorithms with such techniques (example : rare-event
simulations,  , ...). This is a huge implementation effort which also
requires to define a methodology to select the good simulation technique
to be applied.
\item
Statistical model checking algorithms have not yet been applied to the
verification of multi-core systems, this area should be
investigated.
\item
Statistical model checking algorithms do not apply to systems that
combine both stochastic and non deterministic aspects. Extending the
results to such systems is however crucial to perform verification of
security protocols, networking protocols, and performance protocols.
\item
Statistical model checking algorithms reduce to decide between two
hypothesis. In many areas such like systems biology, we may have a
prior knowledge on the probability to satisfy both
hypothesis. Incorporating this prior knowledge in the verification
process may considerably reduce the number of simulations needed for
the algorithm to terminate. A first study has shown impressive gains
in performances \cite{}.
\item
Statistical model checking may help testers! In \cite{MHNC09}, Cavalli
et al. proposed to use statistical techniques for conformance testing
of timed stochastic systems. The technique should be automated. This
could lead to new algorithms for verifying the so-called black-box
systems.
\item
Continuing the work on heterogeneous systems ... 
\end{itemize}

